Interferometric Mapping of Magnetic Fields: The massive star forming region G34.4+0.23 MM

We report millimeter interferometric observations of polarized continuum and line emission from the massive star forming region G34.4. Polarized thermal dust emission at 3 mm wavelength and CO $J=1 \to 0$ line emission were observed using the Berkeley-Illinois-Maryland Association (BIMA) array. Our results show a remarkably uniform polarization pattern in both dust and in CO J=$1 \to 0$ emission. In addition, the line emission presents a consistent uniform polarization pattern over most of the velocity channel maps. These uniform polarization patterns are aligned with the north-south main axis of the filament between the main millimeter source (MM) and the ultra-compact H {\scriptsize II} region, which are the central sources in G34.4, suggesting a magnetic field orthogonal to this axis. This morphology is consistent with a magnetically supported disk seen roughly edge-on.

==> Readme <==
Dear Referee

Thank you very much for your comments that help to improve the quality of our
publication. Your comments on improving the qualitative explanation for the G-K
effect was most helpful, I went through a hard time to understand it during
grad school.

Below you will find detailed answers to all your comments.

Best wishes


Paulo C. Cortes

*****************************
REFEREE'S REPORT

The paper presents interesting and useful new results on the orientation of magnetic fields in star forming regions. It is the latest in a series of papers, by these authors and collaborators, using interferometric observations to obtain high resolution magnetic field data, simultaneously from polarized dust emission and polarized spectral line emission. The results of these observations are extremely important in constraining theories of star formation and the role of magnetic fields in this process: the paper certainly warrants publication in the ApJ. The paper is generally very well written and concise, although a few improvements could be made during copy editing. A few points should also be addressed before publication.

1. The title should describe what type of object G34.4+0.23 MM is!

The title was change to specify the nature of the region.

2. Having a qualitative description of the Goldreich-Kylafis effect in the Introduction is a nice idea to help the reader. However, I found this explanation very difficult to follow, even after drawing diagrams with the directions of various gradients and angular distributions. I had to go to the original G-K papers (and quickly found that these do not contain a qualitative description, which makes me appreciate the authors intentions here more).

A suggestion is to not describe a particular example, but the general principles:
(i) the isotropic unpolarized case,
(ii) the effect of velocity gradients on optical depth,
(iii) the magnetic field gives rise to \sigma and \pi splitting,
(iv) different optical depths of \sigma and \pi results in polarization,
(v) the polarization orientation depends on the relative direction of the velocity gradients and magnetic field.

If the authors wish to retain the current explanation, I think that they should try to write a bit more precisely and use shorter sentences, e.g.:  the clause beginning  "... which will lead to populations of the magnetic M=\pm1 substates..." is superfluous;   another way should be found to say that "...the rate for de-excitation ... is decreased more ...";   at the end "... or perpendicular to the magnetic field." needs to stress "in this example."


I re-wrote the whole paragraph trying to explain with more detail what are the radiaton components
involved and what is the effect of the anisotropies in the competition between these components.
In simple terms, depending on the anisotropies (like LVGs)
 either the pi or sigma components will get higher populations which will lead to
a stronger emission from one of these components. Because this components are polarized
we expect a certain amount of linear polarization to arise.
I tried to follow the referee suggestion about how to state the explanation.


3. In Section 4.1 the integrated fluxes should be given as well as an estimated lower limit. (The measured flux is quoted in Section 5.1 to obtain the core mass.)

The integrated flux was included in Section 4.1. as well as a lower limit. This was very helpful
because I found a typo in the integrated flux which was corrected.

4. In Section 4.2 it is interesting to see that the magnetic field in the outflows probably has the same orientation as in the filament and that the outflows in Fig. 3 do not appear to be perpendicular to the filament. Does this mean that the field is not being distorted or aligned by the outflow? (In another paper in this series the magnetic field was found to be aligned by an outflow.) I think that the authors should, briefly, comment on this.


This is a very interesting issue, the problem is that the BIMA D array configuration give poor
resolution compared with the C array that was used in Cortes2006b. Also G34.4 is at 5 kpc while
NGC2071IR is at 400 pc. The resolution obtained for this paper does not allow us to conclude
anything about the polarization and the outflows in this regions. 
I think that this is even more important for
the dust emission where we may have expected mechanical alignment where the outflows are important.
I hope to get time at any of the current interferometers to do higher resolution observations
to see what is the magnetic field structure in the outflows.

5. In the Summary: what type of observations would be most useful? Information about the field in the filament between the cores?

I added a small paragraph to give more details about this.


I also have a few minor comments on parts of the text.

Section 1, 1st paragraph, 3rd sentence. Should read something like "Magnetic field observations of molecular clouds are divided ...".

changed


Section 1, 1st paragraph, 2nd last sentence. "In this way ... plane of the sky." This sentence is not necessary.

changed

Section 2, about half way through. "The northern component of the core ...". Is this really meant to refer to a component of a core? Or a component of the filament or cloud, or the northern core.

True, a missused of language, it was corrected

Section 4.1, second sentence. What exactly is sigma? The instrumental polarization, system noise, ... (I may be showing my ignorance about this type of observation) and does it take into account positive bias in \sqrt{Q^2 + U^2}.

sigma is the noise for the polarized flux used to set up the cutoff, everything under 3sigma is
cutoff. This value is an input paramter for the impol routine in MIRIAD. The bias is taken care
of by this routine.

Figure 1, caption. The co-ordinates of the G34.4+0.23 MM source should be given, or its position marked on the map.


I added arrows to show the region in Figure 1.

